3D Euler about a 2D Symmetry Plane

Initial results from new calculations of interacting anti-parallel Euler vortices are presented with the objective of understanding the origins of singular scaling presented by Kerr (1993) and the lack thereof by Hou and Li (2006). Core profiles designed to reproduce the two results are presented, new more robust analysis is proposed, and new criteria for when calculations should be terminated are introduced and compared with classical resolution studies and spectral convergence tests. Most of the analysis is on a $512 \times 128 \times 2048$ mesh, with new analysis on a just completed $1024 \times 256 \times 2048$ used to confirm trends. One might hypothesize that there is a finite-time singularity with enstrophy growth like $\Omega \sim (T_c-t)^{-\gamma_\Omega}$ and vorticity growth like $||\omega||_\infty \sim (T_c-t)^{-\gamma}$. The new analysis would then support $\gamma_\Omega \approx 1/2$ and $\gamma > 1$. These represent modifications of the conclusions of Kerr (1993). Issues that might arise at higher resolution are discussed.

==> debug_log_8984 <==

#####Fri Feb 22 13:35:12 2008#####
STARTED admin_physics.miguelb.11925


#####Fri Feb 22 13:35:12 2008#####
------------------------------------------------------------------------------
\\
arXiv:0802.3362
From: Miguel D. Bustamante <mig_busta@yahoo.com>
Date: Fri, 22 Feb 2008 17:46:35 GMT   ()   ()

Title: 3D Euler about a 2D Symmetry Plane
Authors: Miguel D. Bustamante and Robert M. Kerr
Categories: physics.flu-dyn
License: http://arxiv.org/licenses/nonexclusive-distrib/1.0/
Policy: accept
Upload-archive: physics
Upload-subject: hput admin_physics.miguelb.11925
archive: physics is_an_author: 1
\\
  Initial results from new calculations of interacting anti-parallel Euler
vortices are presented with the objective of understanding the origins of
singular scaling presented by Kerr (1993) and the lack thereof by Hou and Li
(2006). Core profiles designed to reproduce the two results are presented, new
more robust analysis is proposed, and new criteria for when calculations should
be terminated are introduced and compared with classical resolution studies and
spectral convergence tests. Most of the analysis is on a $512 \times 128 \times
2048$ mesh, with new analysis on a just completed $1024 \times 256 \times 2048$
used to confirm trends. One might hypothesize that there is a finite-time
singularity with enstrophy growth like $\Omega \sim (T_c-t)^{-\gamma_\Omega}$
and vorticity growth like $||\omega||_\infty \sim (T_c-t)^{-\gamma}$. The new
analysis would then support $\gamma_\Omega \approx 1/2$ and $\gamma > 1$. These
represent modifications of the conclusions of Kerr (1993). Issues that might
arise at higher resolution are discussed.
\\


#warnings_now: ADMIN UPLOAD



#author_warnings_now: 
Author 1: Miguel D. Bustamante
Author 2: Robert M. Kerr
-> Number of authors = 2



#####Fri Feb 22 13:35:12 2008#####
Finished unpacking (errors=)

#author_warnings_now: 
Author 1: Miguel D. Bustamante
Author 2: Robert M. Kerr
-> Number of authors = 2

 physics.miguelb.11925.tar: unpacked 17 files from tar file


#####Fri Feb 22 13:35:12 2008#####
showtime: 0802.3362 being processed as test/9999147 -> /data/ftp/arxiv/papers/0802


#####Fri Feb 22 13:35:12 2008#####
packing to 0802.3362.tar.gz

#####Fri Feb 22 13:35:13 2008#####
running AutoTeX -p test/9999147 -d 0802.3362 at Fri Feb 22 13:35:13 2008

#####Fri Feb 22 13:35:13 2008#####
completed AutoTeX in 0s

#####Fri Feb 22 13:35:13 2008#####
Rejected after unpack_submission()... cleaning up

#warnings_now: ADMIN UPLOAD

Fri Feb 22 13:35:13 2008: AutoTeX took 0s


#####Fri Feb 22 13:35:13 2008#####
About to close and move this log to /u0/incoming/admin_physics.miguelb.11925 which will then be moved to /u0/incoming/rejects

